Weighted Prefix Normal Words: Mind the Gap

A prefix normal word is a binary word whose prefixes contain at least as many 1s as any of its factors of the same length. Introduced by Fici and Lipt\'ak in 2011 the notion of prefix normality is so far only defined for words over the binary alphabet. In this work we investigate a generalisation for finite words over arbitrary finite alphabets, namely weighted prefix normality. We prove that weighted prefix normality is more expressive than binary prefix normality. Furthermore, we investigate the existence of a weighted prefix normal form since weighted prefix normality comes with several new peculiarities that did not already occur in the binary case. We characterise these issues and finally present a standard technique to obtain a generalised prefix normal form for all words overarbitrary, finite alphabets.

==> crazygapfree.tex <==
\begin{definition}
	Let $\mu$ and $\nu$ be \wm s over the same alphabet $\Sigma$ w.r.t. the 
	monoids $(A,\circ)$ and $(B,\times)$.
	We say $\mu$ and $\nu$ are \emph{equivalent} if for all words 
	$v,w\in\Sigma^*$ with $|v|=|w|$ we have $\mu(v)=\mu(w)$ iff $\nu(v)=\nu(w)$ 
	as well as $\mu(v)<_A\mu(w)$ iff $\nu(v)<_B\nu(w)$.
\end{definition}

\begin{corollary}
	The \pn{} form of any word is the same w.r.t. equivalent \wm s.
\end{corollary}

\begin{theorem}
	\label{the:gapfreeEQsum}
	Gapfree \wm s are equivalent to \sumwm s with stepped base weights.
\end{theorem}

The above proposition shows that the monoid and the individual base weights 
used by any gapfree \wm{} do not impact the relative behaviour of the \wm. One 
can simply use a \sumwm{} that has stepped base weights instead. This leads 
us to the definition of the gapfree \emph{standard \wm} that is innate to any 
ordered alphabet.

\begin{definition}
	Let $\Sigma=\{\ta_1,\ta_2,\dots,\ta_n\}$ be a strictly totally ordered 
	alphabet, where $n\in\N$. We define the \emph{standard \wm{}} $\mu_\Sigma$ 
	as the alphabetically ordered \sumwm{} with base weights $\mu(\ta_i) = i$ 
	for all $i\in[n]$.
\end{definition}

\begin{lemma}
	The standard \wm{} is gapfree.
\end{lemma}


\begin{lemma}
	\label{lem:gaptok2}
	Let $\mu$ be a gapfree \wm{} over Sigma w.r.t. the monoid $(A,\circ)$.
	Let $\Sigma = \{\ta_1,\dots,\ta_n\}$ with $n\in\N_{>2}$,
	let $\mu$ be w.l.o.g. injective with 
	$\mu(\ta_i)\prec\mu(\ta_j)$ for all $i<j\in[n]$.
	Then $\mu(\ta_i\ta_{i+2})=\mu(\ta_{i+1}\ta_{i+1})$ for all $i\in[n-2]$.
\end{lemma}
\begin{proof}
	Consider w.l.o.g. the word $u=\ta_3\ta_1\ta_3\ta_2$. Since 
	$f_{u,\mu}(3)=\mu(\ta_3\ta_1\ta_3)$ and $f_{u,\mu}(2)=\mu(\ta_3\ta_2)$ 
	holds and $\mu$ is gapfree we know that there exists some $z\in[n]$ such 
	that $\mu(\ta_1\ta_3)=\mu(\ta_2\ta_z)$.
	
	With $\mu(\ta_1)\prec\mu(\ta_2)\prec\mu(\ta_3)$ if follows that 
	$\mu(\ta_1)\prec\mu(\ta_z)\prec\mu(\ta_3)$ holds.
	So $z=1$ and $\mu(\ta_1\ta_3) = \mu(\ta_1\ta_1)$ hold.
\end{proof}


\begin{proposition}
	Let $\mu$ be a \wm{} over $\Sigma$ w.r.t. the monoid $(A,\circ)$.
	Let $\Sigma = \{a_1,\dots,a_n\}$ with $n\in\N_{>2}$,
	let $\mu$ be (w.l.o.g.) injective with 
	$\mu(a_i)\prec\mu(a_j)$ for all $i<j\in[n]$.
	Now $\mu$ is gapfree if and only if 
	($\mu(a_{i_1}\dots a_{i_k}) = \mu(a_{j_1}\dots a_{j_k}) \iff 
	\sum_{l=1}^{k}i_l = \sum_{l=1}^{k}j_l$ for all $i_l,j_l\in[n]$ for all 
	$l\in[k]$).
\end{proposition}

\begin{proof}
	
$\Leftarrow$). The idea is to use subtraction on sums of indexes to find a 
letter to fill any gap.
Let $w\in\Sigma^*$, $k\in[|w|]$, 
$u\Fact_k(w)$ such that $\mu(u)=f_{w,\mu}(k)$,
and $v\Fact_{k-1}(w)$ such that $\mu(v)=f_{w,\mu}(k-1)$.
Now write $u,v$ as $u=a_{i_1}\dots a_{i_k}$ and $v=a_{j_1}\dots a_{j_{i-1}}$ 
where $i_l\in[n]$ for $l\in[k]$ and $j_l\in[n]$ for $l\in[k-1]$.
Now let $x=\sum_{l=1}^{k}i_l$ and $y=\sum_{l=1}^{k-1}j_l$.
Since $x-y\geq 1$ holds since $\mu(u)>\mu(v)$ holds by choice.
Also $x-y\leq n$ holds since both $u$ and $v$ are chosen with maximum weight.
Assuming the right side of the claim holds there exists a letter $a_{x-y}$ such 
that $f_{w,\mu}(k) = f_{w,\mu}(k-1) \circ \mu(a_{x-y})$ holds, i.e. $\mu$ is 
gapfree.


$\Rightarrow$). Assume $\mu$ is gapfree. Let $k\in\N$ and $w,v\in\Sigma^k$, 
where $w=a_{i_1}\dots a_{i_k}$, $v=a_{j_1}\dots a_{j_k}$, 
$x=\sum_{l=1}^{k}i_l$, and $y=\sum_{l=1}^{k}j_l$ with $i_l,j_l\in[n]$
for all $l\in[k]$.
We show $\mu(w)=\mu(v) \iff x=y$ by induction over $k$.

Case $k=1$: Trivial since $\mu$ is w.l.o.g. injective.

For the following cases w.l.o.g. let $i_1<j_1$, $i_1\leq i_2 \dots i_k$, 
$j_1\leq j_2 \dots j_k$, and $i_l\neq j_{l'}$ for all $l,l'\in[k]$, i.e. 
$w,v$'s letters are ordered by increasing weight and share no letters 
(otherwise we can strike shared letters and apply a case for smaller a $k$ by 
induction).

Case $k=2$: Induction over $i_2-i_1$.

Subcase $i_2-i_1 \in \{0,1\}$: For $i_1=i_2$ we get a $\mu(w)<\mu(v)$ and $x<y$ 
since in that case $i_1<j_1\leq j_2$ holds. Similarly for $i_1+1=i_2$ we get 
$\mu(w)<\mu(v)$ and $x<y$ since in that case $i_1<i_2<j_1\leq j_2$ holds.

Subcase $i_1+2=i_2$: In this case $w=\ta_{i_1}\ta_{i_1+2}$.
Now if $x=y$ holds then $v=\ta_{i_1+1}\ta_{i_1+1}$ since $i_1<j_1\leq 
j_2<i_2=i_1+2$ holds or we get a contradiction otherwise. And with 
Lemma~\ref{lem:gaptok2} we know 
$\mu(\ta_{i_1}\ta_{i_1+2})=\mu(\ta_{i_1+1}\ta_{i_1+1})$ holds.
If on the other hand $\mu(\ta_{i_1}\ta_{i_1+2})=\mu(\ta_{j_1}\ta_{j_2})$ holds 
then again by $i_1<j_1\leq j_2<i_1+2$ we get $j_1=j_2=i_1+1$, i.e. $x=y$.

Subcase $i_2-i_1 > 2$: Let $i_1 + l = i_2$ for some $l\in\N_{>2}$.
Consider $\mu(\ta_{i_1+2}w)=\mu(\ta_{i_1+2}v)$ which is equivalent to 
$\mu(w)=\mu(v)$, and by the previous subcase equivalent to
$\mu(\ta_{i_1+1}\ta_{i_1+1}\ta_{i_1+l})=\mu(\ta_{i_1+2}v)$. Repeat until ...
Use previous subcase to shift weight around for 
inductive argument.

Case $k>2$: follows by using case $k=2$ to swap letters until first letters are 
equal, after removing it we inductively use 
$k-1$. 
	
\end{proof}

==> proof_corNatWM.tex <==
\begin{proof}
The claim follows directly by the structure of $\N$.
\qed
\end{proof}

==> proof_lemALPHWM.tex <==
\begin{proof}
    Follows directly by Proposition~\ref{prop:step1} with
    $\sigma(n)=n+1$ with $n\in\N$.
    \qed
\end{proof}

==> proof_lemGAPTOK2.tex <==
\begin{proof}
	By Induction over $x$. The case for $x=1$ is trivial.
	
	Firstly consider the case $x=2$. 
	W.l.o.g. let $i=1$, so in this case we show that 
	$\mu(\ta_1\ta_3)=\mu(\ta_2\ta_2)$ holds.
	Let $u=\ta_3\ta_1\ta_3\ta_2$. Since $f_{u,\mu}(3)=\mu(\ta_3\ta_1\ta_3)$ and 
	$f_{u,\mu}(2)=\mu(\ta_3\ta_2)$ holds and $\mu$ is gapfree we know that 
	there exists some $z\in[n]$ such that $\mu(\ta_1\ta_3)=\mu(\ta_2\ta_z)$.
	With $\mu(\ta_1)<_A\mu(\ta_2)<_A\mu(\ta_3)$ if follows that 
	$\mu(\ta_1)<_A\mu(\ta_z)<_A\mu(\ta_3)$ holds.
	Therefore $z=2$ and $\mu(\ta_1\ta_3) = \mu(\ta_2\ta_2)$ hold.
	
	Secondly consider $x>2$. Let w.l.o.g $y\leq\lfloor\frac{x}{2}\rfloor$.
	By induction we assume the claim to hold for all smaller $x$, i.e. 
	$\mu(a_{i}a_{i+x-1})=\mu(a_{i+y}a_{i+x-y-1})$ holds and also
	$\mu(a_{j}a_{j+y+1})=\mu(a_{j+1}a_{j+y})$ where $j=i+x-y-1$ holds since 
	$y+1\leq\lfloor\frac{x}{2}\rfloor+1<x$.
	From the first it follows that 
	$\mu(a_{i}a_{i+x-1}a_{i+x})=\mu(a_{i+y}a_{i+x-1-y}a_{i+x})$ holds and with 
	the second rewritten as $\mu(a_{i+x-y-1}a_{i+x})=\mu(a_{i+x-y}a_{i+x-1})$
	it follows that also $\mu(a_{i+y}a_{i+x-1-y}a_{i+x}) = 
	\mu(a_{i+y}a_{i+x-y}a_{i+x-1})$ holds. And together this gives us 
	$\mu(a_{i}a_{i+x})=\mu(a_{i+y}a_{i+x-y})$.
	\qed
\end{proof}


==> proof_propSTEP2.tex <==
\begin{proof}
    W.l.o.g let $\mu$ be injective and 
    let $\Sigma$ be of the form
    $\{\ta_0, \ta_1, \dots , \ta_{n-1}\}$,
    where the letters are in ascending order of their weight,
    so $\mu(\ta_i)\prec\mu(\ta_j)$ holds
    for all $i<j$, $i,j\in[0,n-1]$. 
    
    We prove inductively the existence of $s\in A$ by extending a word that contains the possible combinations of letters that define $f_{w,\mu}$.
    Consider the word
    $w=\ta_1\ta_2\ta_0\ta_2\in\Sigma^*$.
    Then $f_{w,\mu}(2) = \mu(\ta_1\ta_2)$ and
    $f_{w,\mu}(3) = \mu(\ta_2\ta_0\ta_2)$ both hold.
    Assuming $\mu$ is gapfree there exists 
    some $\ta_x\in\Sigma$ with $x\in[0,n-1]$ for which 
    $\mu(\ta_2\ta_0\ta_2) = \mu(\ta_1\ta_2)
    \circ \mu(\ta_x)$ holds.
    Consequently $\mu(\ta_2\ta_0) = \mu(\ta_1\ta_x)$ holds.
    And together with 
    $\mu(\ta_0)\prec\mu(\ta_1)\prec\mu(\ta_2)$
    follows that 
         $\mu(\ta_0)\prec\mu(\ta_x)\prec\mu(\ta_2)$
          holds.
    In other words we now have $0<x<2$.
    So $x=1$ and $\mu(\ta_2\ta_0) = \mu(\ta_1\ta_1)$ hold.
    Now by the additional prerequisite there 
    exists an $s\in A$ such that
    $\mu(\ta_1) = \mu(\ta_0) \circ s$
    and so $\mu(\ta_2\ta_0) = \mu(\ta_1\ta_0)\circ s$ holds.
    Consequently also 
    $\mu(\ta_2) =\mu(\ta_1)\circ s$ holds.
    
    So we already know that $\sigma(a) = a \circ s$ is 
    the step function we need. 
    And finally, by inductively repeating the argument 
    from above for the words
    $\ta_{1+i}\ta_{2+i}\ta_{0+i}\ta_{2+i}\in\Sigma^*$
    for all $i\in[1,n-3]$ it follows that 
    $\mu$ has stepped base weights with the 
    step function $\sigma$.
    For instance, from $\mu$ being gapfree over the word
    $\ta_{2}\ta_{3}\ta_{1}\ta_{2}\in\Sigma^*$
    it follows that also $\mu(\ta_3) =\mu(\ta_2)\circ s$ holds.
    \qed
\end{proof}

==> proof_theGAPEQSTD.tex <==
\begin{proof}
	Let $\mu$ be a gapfree, injective, and alphabetically ordered \wm{} over 
	$\Sigma$ w.r.t. the monoid $A$.
	Let $\Sigma$ by strictly totally ordered and w.l.o.g. let
	$\Sigma = \{a_1,\dots,a_n\}$ with $n\in\N_{>2}$.
	Let $k\in\N$ and $v=\ta_{i_1}\dots\ta_{i_k}\in\Sigma^k$ and 
	$w=\ta_{j_1}\dots\ta_{j_k}\in\Sigma^k$ for all $i_l,j_l\in[n]$ and 
	$l\in[k]$.
	Now $\mu_\Sigma(v)=\sum_{l=1}^{k}i_l$ and $\mu_\Sigma(w)=\sum_{l=1}^{k}j_l$ 
	hold.
	
	We show $\mu(v) <_A \mu(w) \Leftrightarrow \mu_\Sigma(v) < \mu_\Sigma(w)$ 
	holds by induction over $k$:
	
	Case $k=1$: Tivial since $\mu$ and $\mu_\Sigma$ are alphabetically ordered.
	
	For the further cases assume w.l.o.g. that $v$ and $w$ share no letters and 
	let their letters be ordered increasingly, i.e. let $i_l\leq i_{l+1}$ and 
	$j_l\leq j_{l+1}$ for all $l\in[k-1]$, furthermore let $i_1<j_1$.
	
	Case $k>2$: We consider two subcases dependent on $i_k$ and $j_1$. Notice 
	$j_1=i_k$ can not occur since $v$ and $w$ share no letters.
	
	Subcase $i_k<j_1$: In this case we know $i_l<j_{l'}$ for all $l,l'\in[k]$. 
	Therefore $\mu(v)<_A\mu(w)$ and $\mu_\Sigma(v)<_A\mu_\Sigma(w)$ both hold 
	immediately.
	
	Subcase $j_1<i_k$: In this case we choose $x=i_k-i_1$ and $y=j_1-i_1$, 
	consequently $y<x$ holds. Now with Lemma~\ref{lem:gaptok2} we have 
	$\mu(v)=\mu(\ta_{i_1}\dots\ta_{i_{k-1}}\ta_{i_1+x})=
	\mu(\ta_{i_1+y}\ta_{i_2}\dots\ta_{i_{k-1}}\ta_{i_1+x-y})$. 
	The claim follows since $i_1+y=j_1$ and by an inductive assumption
	$\mu(v')<_A\mu(w') \Leftrightarrow \mu_\Sigma(v')<\mu_\Sigma(w')$ holds for 
	$v'=v[2\dots k]$ and $w'=w[2\dots k]$.
	\qed
\end{proof}

%
%We show $\mu(w)=\mu(v) \iff x=y$ by induction over $k$.
%
%Case $k=1$: Trivial since $\mu$ is w.l.o.g. injective.
%
%For the following cases w.l.o.g. let $i_1<j_1$, $i_1\leq i_2 \dots i_k$, 
%$j_1\leq j_2 \dots j_k$, and $i_l\neq j_{l'}$ for all $l,l'\in[k]$, i.e. 
%$w,v$'s letters are ordered by increasing weight and share no letters 
%(otherwise we can strike shared letters and apply a case for smaller a $k$ 
%by 
%induction).
%
%Case $k=2$: Induction over $i_2-i_1$.
%
%Subcase $i_2-i_1 \in \{0,1\}$: For $i_1=i_2$ we get a $\mu(w)<\mu(v)$ and 
%$x<y$ 
%since in that case $i_1<j_1\leq j_2$ holds. Similarly for $i_1+1=i_2$ we 
%get 
%$\mu(w)<\mu(v)$ and $x<y$ since in that case $i_1<i_2<j_1\leq j_2$ holds.
%
%Subcase $i_1+2=i_2$: In this case $w=\ta_{i_1}\ta_{i_1+2}$.
%Now if $x=y$ holds then $v=\ta_{i_1+1}\ta_{i_1+1}$ since $i_1<j_1\leq 
%j_2<i_2=i_1+2$ holds or we get a contradiction otherwise. And with 
%Lemma~\ref{lem:gaptok2} we know 
%$\mu(\ta_{i_1}\ta_{i_1+2})=\mu(\ta_{i_1+1}\ta_{i_1+1})$ holds.
%If on the other hand $\mu(\ta_{i_1}\ta_{i_1+2})=\mu(\ta_{j_1}\ta_{j_2})$ 
%holds 
%then again by $i_1<j_1\leq j_2<i_1+2$ we get $j_1=j_2=i_1+1$, i.e. $x=y$.
%
%Subcase $i_2-i_1 > 2$: Let $i_1 + l = i_2$ for some $l\in\N_{>2}$.
%Consider $\mu(\ta_{i_1+2}w)=\mu(\ta_{i_1+2}v)$ which is equivalent to 
%$\mu(w)=\mu(v)$, and by the previous subcase equivalent to
%$\mu(\ta_{i_1+1}\ta_{i_1+1}\ta_{i_1+l})=\mu(\ta_{i_1+2}v)$. Repeat until ...
%Use previous subcase to shift weight around for 
%inductive argument.
%
%Case $k>2$: follows by using case $k=2$ to swap letters until first letters 
%are 
%equal, after removing it we inductively use 
%$k-1$. 



==> proof_theSIMWM.tex <==
\begin{proof}
    Let $\mu$ and $\nu$ be alphabetically
    ordered, natural, gapfree \wm s over the 
    strictly totally ordered alphabet
    $\Sigma=\{\ta_0,\ta_1,\dots,\ta_{n-1}\}$
    for some $n\in\N$ and with $\mu(\ta_i)<\mu(\ta_j)$
    for all $i<j$, $i,j\in[0,n-1]$.
    And let $v,w\in\Sigma^*$ with $|v|=|w|$.
    Then $\mu$ and $\nu$ are both 
    injective because
    they both are alphabetically ordered.
    
    In case $\Sigma$ is binary, so are
    $\mu$ and $\nu$.
    Therefore if $\mu(v)=\mu(w)$ holds
    $|v|_{\ta_0}=|w|_{\ta_0}$ and 
    $|v|_{\ta_1}=|w|_{\ta_1}$ must hold,
    and so we have $\nu(v)=\nu(w)$.
    The converse and the same for "$<$" hold analogously. 
    
    In the non-binary case both $\mu$ and $\nu$
    have stepped base weights by Proposition~\ref{prop:step2}.
    Thus two step functions $\sigma_\mu$ for $\mu$ and 
    $\sigma_\nu$ for $\nu$ exist.
    Notice, the number of steps in any 
    letter $\ta_i\in\Sigma$ is always $i$ for 
    both of those step functions.
    Therefore the weights of all words have the
    same number of steps in their weight regardless of 
    which one of the two \wm s is considered.
    Now assume $\mu(v)=\mu(w)$ holds, then 
    both words have the same number of 
    steps in their $\mu$-weight.
    Thus also their $\nu$-weight must have this
    number of steps and so $\nu(v)=\nu(w)$ holds.
    Again the converse and the same for "$<$" hold analogously.
    \qed
\end{proof}

==> sec-giwm.tex <==
%%%%%%%%%%%%%%%%%%
%%%%%%%%% OLD
%%%%%%%%%%%%%%%%%%%%%%%

In this section we investigate the behaviour of
gapfree and injective \wm s in more detail.
First of all, by their definition
we can infer that every binary \wm{} is gapfree and
\pwm s are in general gapful.

\begin{lemma}
    \label{lem:binwm}
    All binary \wm s are gapfree.    
\end{lemma}
\ifpaper % ONLY PAPER
\else    % ONLY ARCHIVE
\input{proof_lemBinWms}
\fi

\begin{remark}
    By Lemma~\ref{lem:binwm}, we see that when modelling binary \pnity{} by means
    of weighted \pnity{} (e.g. in the proof of Theorem~\ref{the:weight2bin})
    we have the existence of a unique binary \pn{} form as expected.
\end{remark}


Following Remark~\ref{rem:pwm} the \pwm s might prove interesting regarding the 
\emph{Indexed JPM} (IJPM).
We found the weight of a word under a \pwm{} to be characteristic for
its Parikh vector via the prime factorisation.
However, we saw that for some words the
\pn{} form has a different Parikh vector,
which is prohibited by \pwm s.
Consequently every \pwm{} has gaps
over such words and is therefore gapful.

\begin{lemma}
    \label{lem:primeWM}
    All non-binary \pwm s are gapful.
\end{lemma}
\ifpaper % ONLY PAPER
\else    % ONLY ARCHIVE
\input{proof_lemPrimeWM}
\fi

In the last section we saw that we have exactly one
weighted \pn{} form in a \factorWEqnce{} class
if the \wm{} is injective and gapfree.
We now give an alternative condition under
which a \wm{} is gapfree.
In most cases this condition is easier 
to prove than the original
statement on gapfree \wm s.
We will also see that this condition is a proper 
characterisation for gapfree \wm s w.r.t.
certain kinds of monoids.

\begin{definition}
    \label{def:sbw}
    Let $(A,\circ)$ be a strictly totally ordered monoid.
    A \emph{step function} is a function $\sigma:A\to A$
    for which there exists an $s\in A$ (the \emph{step})
    such that we have $\sigma(a) = a\circ s$ for all $a\in A$.
    The \wm{} $\mu$ over $\Sigma$ w.r.t the monoid $A$
    has \emph{stepped base weights} if
    there exists a step function $\sigma$
    such that $\mu(\Sigma)=\{ \sigma^i(\min(\mu(\Sigma)))
    \mid i\in[0,|\mu(\Sigma)|-1]\}$ holds.
\end{definition}

% WIP TODO
\begin{remark}
    \label{rem:stepWM2}
    For understanding that indeed steps greater than $1$,
    and thus a monoid different from $(\N,+)$, are justified,
    consider $(\mu(\Sigma^{\ast}),+)$ not being isomorphic to $(\N,+)$.
    In this case, words can be constructed which have a different weight
    in $\N$ than the sum of their letters.
\end{remark}


In the previous example for $\Sigma =\{\ta,\tb,\tc\}$ the
\wm{} $\mu$ over $\Sigma$ with $\mu(\ta) = 2$, $\mu(\tb) = 4$,
and $\mu(\tc) = 6$ has stepped base weights with the step of $2$.
In contrast the \sumwm{} $\nu$ over $\Sigma$ with 
$\nu(\ta) = 1$, $\nu(\tb) = 3$, and $\nu(\tc) = 4$ does not,
because $\nu(\tb) - \nu(\ta) = 2$
but $\nu(\tc) - \nu(\tb)=1$.


The following two propositions characterise the 
relation between gapfree \wm s and those with stepped base weights.

\begin{proposition}
    \label{prop:step1}
    All \wm s with stepped base weights are gapfree.
\end{proposition}
\ifpaper % ONLY PAPER
\else    % ONLY ARCHIVE
\input{proof_propSTEP1}
\fi

For the converse statement to hold we unfortunately need 
the additional prerequisite that there exist 
elements in the chosen 
monoid that are able to fulfil the 
property of stepped base weights.
For every two weights $a<b$ we need an element $x$ 
such that $b=a\circ x$ holds.
To see that this is necessary,
consider for example the alphabet
$\Sigma=\{\ta,\tb,\tc\}$ and the 
strictly totally ordered monoid 
$(A,\circ)$ 
where $A$ is the set $\{\colvec{a\\b} \mid a,b\in\N_0 \}$,
$\circ$ is the usual addition on vectors,
$\neutr_A = \colvec{0\\0}$,
and $<_A$ is the order obtained 
by the lexicographical extension of the usual 
order on integers onto vectors.
So for example $\colvec{0\\0}<_A\colvec{0\\2}
<_A\colvec{1\\1}<_A\colvec{2\\0}$ holds.
Now the \wm{} $\mu$ over $\Sigma$ with the base weights
$\mu(\ta) = \colvec{0\\2}$, $\mu(\tb) = \colvec{1\\1}$ and 
$\mu(\tc) = \colvec{2\\0}$ is gapfree but has no stepped base weights.

\ifpaper
\else
\begin{proposition}
    \label{prop:fancymonoid}
    Let $\Sigma=\{\ta,\tb,\tc\}$ and let 
    $(A,\circ,\neutr_A, <_A)$ be the strictly totally ordered monoid
    where $A=x<\{\colvec{a\\b} \mid a,b\in\N_0 \}$,
    $\circ$ is the usual addition on vectors,
    $\lambda = \colvec{0\\0}$,
    and $<_A$ is the order obtained 
    by the lexicographical expansion of the usual 
    \emph{less than} onto vectors,
    e.g $\colvec{0\\0}<_A\colvec{0\\2}
    <_A\colvec{1\\1}<_A\colvec{2\\0}$ holds.
    The \wm{} $\mu$ over $\Sigma$ with base weights
    $\mu(\ta) = \colvec{0\\2}$,
    $\mu(\tb) = \colvec{1\\1}$, and 
    $\mu(\tc) = \colvec{2\\0}$ is gapfree.
\end{proposition}
\fi
The idea of the proof is the following: let $u\in\Fact_{i+1}(w)$ and
$v\in\Fact_{i}(w)$ such that $\mu(u) = f_{w,\mu}(i+1)$ and 
$\mu(v) = f_{w,\mu}(i)$.
If $v$ is a prefix or a suffix of $u$,
the claim holds immediately.
Thus, consider that $v$ is neither a prefix nor suffix of $u$;
indeed we can also assume that they do not overlap in $w$ since
the overlap would count for $\mu(u)$ and $\mu(v)$ in the same way.
If we fix the different amount of $\ta$ and $\tc$ between $v$ and $u$,
namely $r$ and $t$, the amount of $\tb$ in both $u$ and $v$
is given by their length and therefore we assume $|u|_{\tb}=0$.
Now by combining $\mu(u)\succ\mu(v)$, $\mu(v)\succ\mu(u[1..|u|-1]),\mu(u[2..|u|])$,
and $|v|+1=|u|$ we get that $t-r\in\{-1,0\}$.
Evaluating both cases gives us 
$f_{w,\mu}(i+1)=f_{w,\mu}(i)+\mu(\ta)$ and
$f_{w,\mu}(i+1)=f_{w,\mu}(i)+\mu(\tb)$ respectively. 
But even though $\mu$ is gapfree,
$\mu(\Sigma) = \{\colvec{0\\2}, \colvec{1\\1}, \colvec{2\\0}\}$
can never be of the form 
$\{\sigma^i(\colvec{0\\0}) \mid i\in[0,2]\}$
for any step function
$\sigma(a)=a\circ \colvec{x\\y}$.
This is the case because there exists 
no $\colvec{x\\y}\in A$ such that
$\colvec{1\\1} = \colvec{0+x\\2+y}$,
$\colvec{2\\0} = \colvec{1+x\\1+y}$, or
$\colvec{2\\0} = \colvec{0+x\\2+y}$ would hold. A full proof can be found in the appendix.

\ifpaper
\else
\input{fancymonoid}
\fi


\begin{proposition}
    \label{prop:step2}
    Let $\mu$ be a non-binary \wm{} over $\Sigma$ w.r.t. the monoid $(A,\circ)$ 
    such that for all $\ta,\tb\in\Sigma$ with $\mu(\ta)<_A\mu(\tb)$ there 
    exists an $s\in A$ such that $\mu(\tb) = \mu(\ta) \circ s$.
    Now if $\mu$ is gapfree then it has stepped base weights.
\end{proposition}
\ifpaper % ONLY PAPER
\else    % ONLY ARCHIVE
\input{proof_propSTEP2}
\fi

\begin{corollary}
    \label{cor:natWm}
    For all natural, non-binary \wm s the additional property of Proposition~\ref{prop:step2} holds.
    Consequently such a \wm{} is gapfree if and only if
    it has stepped base weights.
%    there exists a step function $\sigma$ with 
%    $\mu(\Sigma)=\{ \sigma^i(\min(\mu(\Sigma))) \mid i\in[0,|\mu(\Sigma)|-1]\}$.
\end{corollary}
\ifpaper % ONLY PAPER
\else    % ONLY ARCHIVE
\input{proof_corNatWM}
\fi


By this characterisation we get 
a generalisation for gapfree \wm s.

\begin{theorem}
    \label{the:simwm}
    For a strictly totally ordered alphabet $\Sigma$, all \wm s
    that are natural, alphabetically 
    ordered, and gapfree behave similarly to one another,
    i.e. for two such \wm s $\mu$ w.r.t. monoid $A$ and $\nu$ w.r.t. monoid $B$ 
    and all words 
    $v,w\in\Sigma^*$ with $|v|=|w|$ we have
    $\mu(w) = \mu(v)$  iff $\nu(w) = \nu(v)$ as well as
    $\mu(w) <_A \mu(v)$ iff $\nu(w) <_B \nu(v)$.
\end{theorem}
\ifpaper % ONLY PAPER
\else    % ONLY ARCHIVE
\input{proof_theSIMWM}
\fi

Theorem~\ref{the:simwm} essentially shows that
the monoid and the individual base weights of any natural,
alphabetically ordered, and gapfree \wm{} do not impact 
the relative behaviour of such \wm s.
This especially includes that
the \pn{} form of any word is the 
same w.r.t. different such natural, alphabetically 
ordered, and gapfree \wm s.
This behaviour leads us to the definition of an \emph{innate} \wm{}
that only depends on the alphabetic order of the letters.

\begin{definition}
    Let $\Sigma=\{\ta_1,\ta_2,\dots,\ta_n\}$
    be a strictly totally ordered alphabet, where $n\in\N$.
    We define the \emph{alphabetic \wm{}} for $\Sigma$ $\mu_\Sigma$ as the alphabetically ordered
    \sumwm{} with base weights $\mu(\ta_i) = i$ for all $i\in[n]$.
\end{definition}

\begin{lemma}
    \label{lem:alphwm}
    The alphabetic \wm{} is gapfree.
\end{lemma}
\ifpaper % ONLY PAPER
\else    % ONLY ARCHIVE
\input{proof_lemALPHWM}
\fi

\begin{conjecture}\label{conj}
    We conjecture that the statement of Theorem~\ref{the:simwm} holds not only for 
    natural, alphabetically ordered, and gapfree \wm s (or \wm s with the aforementioned 
    composition property) but also for any alphabetically 
    ordered, gapfree \wm s.
\end{conjecture}

In the remaining part of this section we investigate 
non-injective \wm s,
specifically we provide a construction that
can be used to transform any \wm{} into an injective one.
This enables us to consider injective \wm s
w.l.o.g most of the time.

\begin{definition}
    \label{def:projWM}
    Let $\mu$ be a \wm{} over $\Sigma$
    w.r.t. the monoid $A$.    
    We define the \emph{$\mu$-projected alphabet} 
    $\Sigma_\mu:= \{ [\ta]_\mu \mid \ta \in\Sigma\} \text{,} $
    where $[\ta]_\mu=\{ \tb\in\Sigma\mid \mu(\tb)=\mu(\ta) \}$
    for $\ta\in\Sigma$ and set $\mu$'s \emph{projected \wm{}} as the 
    \wm{} $\hat{\mu}$ over $\Sigma_\mu$ w.r.t. $A$
    with the base weights
    $\hat{\mu}([\ta]_\mu) = \mu(\ta)\text{.}$
    Finally for a word $w\in\Sigma^*$ we construct its \emph{$\mu$-projection}
    $w_\mu\in\Sigma_\mu^*$ with 
    $w_\mu:=[w[1]]_\mu\dots[w[|w|]]_\mu \text{.}$
\end{definition}

\begin{lemma}
    \label{lem:makeInjective}
    For a weight measure $\mu$ over an alphabet $\Sigma$
    and a word $w\in\Sigma^*$ we have $\hat{\mu}(w_\mu)=\mu(w)$
    and the projected \wm{} $\hat{\mu}$ is injective on $\Sigma_\mu$.
\end{lemma}
\ifpaper % ONLY PAPER
\else    % ONLY ARCHIVE
\input{proof_lemMakeInj}
\fi

%%%%Duplicate from below
%For example again consider the sum weight measure
%$\mu$ over $\Sigma=\{\ta,\tn,\tc,\tb\}$
%with base weights $\mu(\ta) = 1$, $\mu(\tn) = \mu(\tc) = 2$, and $\mu(\tb) = 3$.
%Then $\mu$'s projected \wm{} $\hat{\mu}$ is a \wm{} over the alphabet
%$\Sigma_\mu=\{\{\ta\},\{\tn,\tc\},\{\tb\}\}$
%with base weights
%$\hat{\mu}(\{\ta\}) = 1$,
%$\hat{\mu}(\{\tn,\tc\}) = 2$, and
%$\hat{\mu}(\{\tb\}) = 3$
%and we see that $\hat{\mu}$ is injective over $\Sigma_\mu$.
    
\begin{remark}
    With this construction a word $w$ and its $\mu$-projection
    $w_\mu$ behave the same way under any 
    function that is based on the weights of 
    the letters in the words, e.g. 
    $f_{w,\mu} = f_{w_\mu,\hat{\mu}}$,
    $p_{w,\mu} = p_{w_\mu,\hat{\mu}}$,
    $\maxpos_{w,\mu} = \maxpos_{w_\mu,\hat{\mu}}$,
    and $\minpos_{w,\mu} = \minpos_{w_\mu,\hat{\mu}}$ all hold.
    Analogously, all other statements depending on those
    functions hold for the $\mu$-projection of the words as well.
    Thus, $w_\mu$ represents all words within
    the set $\{v\in\Sigma^* \mid v[i]\in w[i] \text{ for all } i\in[|w|]\}$.
\end{remark}

The following theorem essentially shows that 
the \pn{} form of a projected word 
like in Definition~\ref{def:projWM}
represents the set of \pn{} words that are
\factorWEqnt{} to the original word.
In other words, for some $w\in\Sigma^*$ the sets
$\mathcal{P}_\mu(w)$ and $\mathcal{P}_{\hat{\mu}}(w_\mu)$
represent the same \pn{} words over $\Sigma$ 
that are equivalent to $w$.
Thus, also in the non-injective case
we are able to obtain one \pn{} form 
by considering projections.

\begin{theorem}
    \label{the:PiP}
    Let $\mu$ be a gapfree \wm{} over $\Sigma$ w.r.t.
     the monoid $A$ and let $w\in\Sigma^*$.
    Then with $w'\in \mathcal{P}_{\hat{\mu}}(w_\mu)$ we have
    $\mathcal{P}_\mu(w)
    = \{ v\in\Sigma^* \mid v[i]\in w'[i] \text{ for all }i\in[|w|] \}$.
\end{theorem}
\ifpaper % ONLY PAPER
\else    % ONLY ARCHIVE
\input{proof_thePiP}
\fi


With Theorem~\ref{the:PiP} we can also
accurately calculate the cardinality of $\mathcal{P}_\mu(w)$
for some word $w\in\Sigma^*$ and a non-injective \wm{} $\mu$.

\begin{corollary}
    \label{cor:count}
    Let $\mu$ be a gapfree \wm{} 
    over the alphabet $\Sigma$,
    $w\in\Sigma^*$, and $w'=\mathcal{P}_{\hat{\mu}}(w_\mu)$.
    Then $|\mathcal{P}_\mu(w)|=\prod^{|w|}_{i=1}|w'[i]|$ holds.
\end{corollary}
\ifpaper % ONLY PAPER
\else    % ONLY ARCHIVE
\input{proof_corCountP}
\fi

We conclude this section by revisiting an example w.r.t.
the projected weight measure.
Again consider the \sumwm{} $\mu$ over $\Sigma=\{\ta,\tn,\tc,\tb\}$
with the base weights $\mu(\ta) = 1$, $\mu(\tn) = \mu(\tc) = 2$, and $\mu(\tb) = 3$.
Then $\mu$'s projected \wm{} $\hat{\mu}$
is a \wm{} over the alphabet
$\Sigma_\mu=\{\{\ta\},\{\tn,\tc\},\{\tb\}\}$ with the base weights
$\hat{\mu}(\{\ta\}) = 1$,
$\hat{\mu}(\{\tn,\tc\}) = 2$, and
$\hat{\mu}(\{\tb\}) = 3$ and we see that $\hat{\mu}$ is injective on $\Sigma_\mu$.
We already know that $\mathtt{nanaba}$ has
multiple \factorWEqnt{} words that are \pn{},
specifically we have
$\mathcal{P}_\mu(\mathtt{nanaba})=
\{\mathtt{banana},\mathtt{bacana},\mathtt{banaca},\mathtt{bacaca}\}$.
Thus, we have the the \pn{} form
$\{\tb\}\{\ta\}\{\tn,\tc\}\{\ta\}\{\tn,\tc\}\{\ta\}$
of 
$(\mathtt{nanaba})_\mu=\{\tn,\tc\}\{\ta\}\{\tn,\tc\}\{\ta\}\{\tb\}\{\ta\}$.
All \factorWEqnt{} and \pn{} words are represented by
this word when reading it as a non-deterministic concatenation of letters,
like shown in Theorem~\ref{the:PiP}, i.e., we have $\mathcal{P}_\mu(\mathtt{nanaba})
= \{ v\in\Sigma^* \mid v[i]\in \mathcal{P}_{\hat{\mu}}((\mathtt{nanaba})_\mu)[i], i\in[6] \}$.




